SDNFV: Flexible and Dynamic Software Defined Control of an Application- and Flow-Aware Data Plane

Software Defined Networking (SDN) promises greater flexibility for directing packet flows, and Network Function Virtualization promises to enable dynamic management of software-based network functions. However, the current divide between an intelligent control plane and an overly simple, stateless data plane results in the inability to exploit the flexibility of a software based network. In this paper we propose SDNFV, a framework that expands the capabilities of network processing-and-forwarding elements to flexibly manage packet flows, while retaining both a high performance data plane and an easily managed control plane. SDNFV proposes a hierarchical control framework where decisions are made across the SDN controller, a host-level manager, and individual VMs to best exploit state available at each level. This increases the network's flexibility compared to existing SDNs where controllers often make decisions solely based on the first packet header of a flow. SDNFV intelligently places network services across hosts and connects them in sequential and parallel chains, giving both the SDN controller and individual network functions the ability to enhance and update flow rules to adapt to changing conditions. Our prototype demonstrates how to efficiently and flexibly reroute flows based on data plane state such as packet payloads and traffic characteristics.

==> discuss.tex <==

\section{Discussion}

A key decision in SDNFV's architecture was how to partition the control of functions between the individual VM, the Flow Controller, and the SDN Controller. We see the need to take advantage of local information where appropriate,
% the autonomy that can be provided to the individual components as needed,
while ensuring that decisions requiring network-wide visibility or that have network-wide impact are performed by an entity with all requisite information. Finally, a key criterion for us is to ensure efficient operation, with little or no degradation to line-rate packet processing.
% All of these considerations go into which component may update the flow tables in the host for managing flows.

% The individual VMs have information regarding the packet flows they process, as well as application context.
Individual VMs can understand packet sequences and their relationship to application and protocol state, and it may be infeasible or inefficient to have that information passed to the SDN Controller, or even to the Flow Controller in the host. Moreover, the VM may want to make local, autonomous decisions regarding the flow and update entries in the flow table. For example, a VM may determine that this flow requires additional QoS monitoring (e.g., a proxy that seeks to optimize content, such as video, for an end-user).

The Flow Controller has visibility into the state across flows being procssed at all VMs within its host. Thus the Flow Controller may have enough information to autonomously update the local flow table, without necessarily contacting the SDN Controller. For instance, when a set of VMs indicate that a flow (or flows, say from a set of source address prefixes) has shown anomalous behavior,  the Flow Controller could set up the flow table to have packets of the flow delivered in parallel to an additional network function for deep packet inspection.

Finally, the state at a VM and across VMs and in the platform could be passed up to the SDN Controller for it to make the decision to update the flow table, including having packets of the flow diverted to a different inteface/next hop. The SDN Controller should be invoked when decisions that have network wide impact have to be performed. Moreover, it may also be done when the decision depends on the state or information collected at multiple nodes in the network.

By having the ability to make informed decisions to update the flow tables at each of these points in the network, we are able to balance between the autonomy enabled at each NFV node in the network, while also ensuring the need to have the logically central controller participate in decisions that have network wide impact.

% To mediate all the access to the flow table across the various components, we find it desirable to have the Flow Controller be used in that role. This would be the case also for the interactions between the VMs and the SDN Controller. We don't forsee the Flow Controller being a bottleneck as the amount of operations that have to be channeled through the Flow Contoller are likely to be small.

% We believe that running network functions in VMs is a crucial design decision. VMs have overwhelmingly become the preferred way to run server applications because of the ease of deployment and resource management that they provide.  VMs also make it easy to encapsulate a software environment to provide virtual ``appliances'' which users can easily setup without having to worry about library dependencies or conflicts. By allowing network functions to be deployed as appliances, we believe that SDNFV will enable the developer community to build a wide range of network services that can all be easily integrated and deployed.


==> extra.tex <==
\section{Extra text}
\note{This text used to be in \ref{sec:decisions}---it is somewhat repetitive with the intro and background.  What should we keep, and where?}

In the current ``simple data plane'' paradigm, it is the SDN Controller's job to determine how flows are routed. While this lets the controller make decisions based on its view of global state, it quickly becomes the bottleneck if decisions cannot be made a priori or based solely on the first packet in each flow.  Clearly, implementing the Video Flow Detector or IDS NFs as modules in an SDN controller would be far too costly since it would require deep analysis of multiple packets for each flow.

The other extreme is to allow individual NFs to make all flow routing decisions (perhaps after some initial input from the SDN controller). In such a case, each NF would be aware of all other NF components in its application, and decide on a per-packet basis how a flow should be routed. This would provide very fine grained control and allows application-specific data that only NFs can efficiently obtain to be used for decision making.  However, it would also eliminate the benefits of SDNs to provide flow-specific control and management; reverting to a distributed model can make it difficult to provide such fine-grained control and management when there are a large number of NFs.

With SDNFV, we instead take a hierarchical control approach that leverages not only the SDN controller and the NFs, but the NF Manager on each host as well.
The SDNFV Application is responsible for transforming a service graph into a set of initial rules sent by the SDN Controller to the NF Managers. The SDN controller additionally has visibility across network nodes and is responsible for flow routing decisions across multiple nodes in the network. The NF Manager makes generic (i.e., application-agnostic) decisions based on packet headers as well as local state and QoS metrics (NF load/queue levels, available link bandwidth, delay, flow rates, etc) and routes packets to individual NFs. NFs are responsible for making application specific control decisions and doing complex processing that involves data from sequences of packets of an individual flow or across flows. This provides convenient high-level control in the SDNFV Application and SDN Controller, but still leaves both the NF Manager and NFs some freedom in how individual packets are routed.  The key focus of our work is on providing the right abstractions and interfaces to allow this to happen flexibly and efficiently.

\cut{
        \vspace{1mm}
        \begin{noitemize}
        \item SDN Controller determines the default NFs a flow must traverse and {\em where} to route the flow to reach them.

        \item The NF Manager determines {\em which NF instance} of a desired type on the host a flow should be delivered to and makes local, application-agnostic routing decisions such as load balancing.

        \item NFs determine {\em what type of NF} a flow should visit next when the default action is not sufficient, and requests the NF Manager to modify routing rules based on data plane observable state.
        \end{noitemize}
}

==> figures/Latency_Nocomputation_table.tex <==
\begin{table}[h]
\begin{tabular}{llll}
\textbf{\#VM \textbackslash Latency(us)} & \textbf{Avg} & \textbf{Min} & \textbf{Max} \\
0VM(dpdk)                                & 26.66        & 23           & 29           \\
1VM                                      & 27.78        & 24           & 35           \\
2VM(parallel)                            & 28.02        & 24           & 37           \\
3VM(parallel)                            & 28.38        & 24           & 40           \\
2VM(seq-table)                           & 28.86        & 24           & 43           \\
3VM(seq-table)                           & 29.96        & 25           & 49          
\end{tabular}
\end{table}

==> figures/MemSwitch-MaxThoughput.tex <==
\begin{table}[h]
\begin{tabular}{ll}
                      & Max Tput(1K Reqs) \\
TwemProxy(4 byte key) & 90                        \\
NetVM(4 byte key)     & 8113                      \\
NetVM(68 byte key)    & 7113                      \\
NetVM(196 byte key)   & 4882                     
\end{tabular}
\end{table}


==> smartdata.tex <==

\section{Challenges for A Smarter Data Plane}

This section describes the benefits of adding intelligence to the data plane, and the systems challenges that must be overcome to do so. We present a series of use cases where flow management decisions require data-plane intelligence not currently available in SDNs; each offers insight into the design choices behind SDNFV.

% \note{This section should give uses cases that motivate why the data plane needs to have intelligence. It should also clearly specify some challenges that arise because of these needs.  The SIGCOMM OpenNF paper did a good job with this structure... let's do the same.}

%% Performance
%	- minimize overheads for transmitting packets (latency)
%	- scalability for multi-cores
%% Ease of deployment
%	- user space applications
%	- VMs 
%% Complex topologies
%	- support networks of NFs
%	- easy addressing

\subsection{Control Based on Packet Histories}

SDNs achieve efficiency despite having a logically centralized controller by limiting the interactions between the controller and the data plane switches to the first packet of a flow. Having more frequent communication with the controller dramatically decreases the achievable throughput, as was shown in Figure~\ref{fig:background:sdncost}. However, there are many traffic management scenarios where it is desirable to observe a flow for some time before deciding how it should be managed, yet such cases cannot be efficiently supported by today's SDN frameworks. Having a software based network such as what we propose in SDFNV enables such an approach, as we are no longer limited by the simplistic capabilities of a hardware (ASIC) based data forwarding plane.

\vspace{2mm}
\noindent {\bf Ants and Elephants:} Detecting and managing lightweight (ant) and heavyweight (elephant) flows has been a subject of much research in recent years~\cite{Quan:2010:CRL:1879141.1879198}. Flows are typically classified by observing the size and rate of packets over a time interval.  While it is possible to use sampling approaches where only periodic flow statistics (number of packets and number of bytes) are sent to the SDN controller to reduce the overhead of flow classification, this risks misidentifying some flows and places undue burden on the controller. Ideally, a smart data plane should be able to not only gather flow state information, but efficiently apply the classification algorithms to incoming packets.  {\em Thus it is crucial that a network function architecture support packet processing at line rates and be scalable in multi-core environments.}


Once flows have been identified, various traffic management techniques can be applied: heavy flows might be redirected over higher bandwidth links, or light ones may have additional QoS processing performed on them to ensure they aren't starved of capacity.
To build this kind of traffic management system requires coordination across the network's data plane and control plane. 
% The SDN controller cannot be relied upon to characterize flows, instead this should be done by an efficient network function that can gather the desired statistics at line rate and perform periodic processing to identify flows. 
Once a flow is identified, the network function should be able to adjust how subsequent packets are processed, which could involve more network functions on the same and other hosts. {\em Thus a smart data plane must not keep its intelligence in isolation; network functions need to be able to coordinate with the SDN controller to redirect flows to other functions throughout the network based on the flow state they observe.} 


\subsection{Application-aware Data Plane}

Limiting SDN controllers to observe only the headers of the first packet in a flow not only prevents characterizing temporal characteristics, but also can prevent the SDN controller from interpreting application-level information that is only found in the packet's payload.  

%% some of this is from smartswitch paper
\vspace{1mm}
\noindent {\bf Application-aware Proxies:} A proxy is a common data center network service that requires application-level information to make decisions about how packets should be routed.  For example, a web application may use a load balancing proxy in front of a cluster of memcached servers since the number of memcached servers may change dynamically and it is impractical to have the web servers know the mapping of keys to cache servers. These types of application-aware network functions often repurpose code from existing application libraries, {\em thus it is highly desirable for network functions to be implemented in a convenient development environment, i.e., as user space applications, not as difficult to write kernel modules or inflexible hardware implementations.}

A common solution to this problem is to employ a proxy such as TwemProxy or moxi, user space applications that act as a front end to the memcached cluster and redirect requests after determining which key is being requested. However, these proxies lack the throughput capabilities of an efficient network function platform.  They also too-tightly mix the control and data plane, making it difficult to integrate such a proxy into a suite of network functions being applied to a flow and managed by an SDN controller. 
Ideally, {\em network
functions should be aware of the application-level state of a flow, while the SDN controller should have the ability to manage the overall flow at a coarser time scale, while being aware of the application level requirements.}



% -- explain why data plane elements should be aware of application-level state. Goal is for SDN controller to know about overall applications, but let data plane worry about specific state details.

% -- example: memcached/http load balancing


% \subsection{Using State from Multiple Flows}
% -- show that often you need to correlate state across multiple flows to make decisions. You also may need to use server load state to make decisions for load balancing/reliability

% -- examples: 1) load balancing between VMs based on queue length and 2) DDoS detection/mitigation

% \note{??? This is a nice use case, but I'm not sure what challenge it emphasizes.  Maybe we should just use this for the experiment/merge part of this idea into the earlier section on packet histories?}

\subsection{Networks of Network Functions}

As network functions become more efficient, flexible, and software based, we believe that they will see an increasingly wide range of uses in data center networks as well as wide area networks. Networks will rely on complex service chains of NFs that each apply some kind of processing or forwarding decisions to packets in a flow. Thus, we will truly be able to exploit the capabilities of a software based network.

\vspace{1mm}
\noindent {\bf Denial of Service Prevention:} Current DDoS detection and mitigation systems are built from expensive hardware and software combinations.  Since fully analyzing each packet's data to determine if it is malicious is very expensive, they are typically made up of a chain of detection elements of increasing cost and accuracy.  If incoming packet rates are low and no attacks are suspected, then flows may only need to traverse a simple firewall. Once administrators suspect an attack, they may reroute flows through more complex deep packet inspection services that watch for TCP SYN floods or attack traffic that conforms to well-known traffic signatures. Finally, if an attack is at full force, then packets may be further rerouted through a set of packet scrubbers that separate the good from the bad. {\em This example demonstrates how a Network Function (NF) is unlikely to work alone, but will have to be part of a complex, dynamic service chain.
Thus an NF needs to be able to adjust how packets are routed and what services are applied to them, without expensive coordination with the SDN Controller.}

% Further, this use case illustrates how networks need to be able to respond 


\subsection{SDNFV Design Criteria}

% Our approach to Software Defined Network Function Virtualization is based upon the above challenges related to performance, ease of deployment, and support for complex service topologies. 
% The SDNFV platform must:
% \begin{itemize}
% \item allow line rate packet processing with minimal added latency, and provide scalability with multi-core deployments.
% \item facilitate development by supporting network functions written as user space applications, and simplify deployment and interoperability by allowing them to run in VMs.
% \item support network functions that dynamically route flows based on packet sequences from one or more flows, application-level data, and server capacity.
% \item efficiently support complex service topologies that span multiple hosts.
% \item enable flexible coordination between network functions and the SDN controller.
% \end{itemize}


% SDNFV facilitates building complex network services composed of multiple data plane processing elements.  It achieves this by representing the overall service as a graph of network functions which are then implemented inside user space applications in a set of VMs spread across one or more hosts.  The SDNFV platform then forwards packets between VMs, providing scalable throughput by pipelining processing functions and optimizing latency by allowing multiple functions to act on a flow in parallel where possible.  Finally, the network function components may need to update the SDN application state based on data plane information, so SDNFV allows VMs to update local flow table state and connect to the SDN controller application. 
Based on these example use cases and the challenges they pose, we have designed our SDNFV platform to meet the following criteria. SDNFV must:

\vspace{1mm}
\noindent 1. {\em Allow line rate packet processing with minimal latency, and provide scalability in multi-core deployments.}

We achieve this goal by building our platform on a zero-copy, lockless, polling-based packet processing framework. This minimizes overheads when moving packets between network functions, and allows for maximal scalability by eliminating all critical sections. SDNFV further optimizes for latency by allowing multiple read-only NFs to process a packet stream in parallel (\S \ref{sec:arch:parallel}), by caching flow table lookups, and automatically load balancing across cores (\S \ref{sec:arch:optimizations}).

\vspace{1mm}
\noindent 2. {\em Efficiently support complex network function service chains spanning multiple hosts}.

SDNFV enables this by representing the overall network service as a graph of network functions which are then implemented inside a set of VMs spread across one or more hosts (\S \ref{sec:arch:servicegraphs}). The SDNFV controller configures flow table rules on the NF Hosts and regular switches in order to properly route flows to the designated services.


\vspace{1mm}
\noindent 3. {\em Permit network functions to dynamically route flows, and enable flexible coordination between network functions and the SDN controller.}

Our platform coordinates with the SDN controller to determine the initial flow table rules (\S \ref{sec:arch:flowtable}), but allows VMs to update local flow table state and connect to the SDN controller application (\S \ref{sec:arch:sndcoord}). This allows SDNFV to support smart data plane functions that dynamically route packets based on temporal characteristics of one or more flows, application-level packet data, or server state such as NF queue lengths.

\vspace{1mm}
\noindent 4. {\em Facilitate development by supporting network functions as user space applications, and simplify deployment and interoperability by running them in VMs.}

SDNFV runs network functions in VMs based on the KVM platform. NFs can be easily written as user space applications using our SDNFV-User Library that provides hooks to process packets and helper functions for common packet manipulations (\S \ref{sec:arch:nfs}).


==> state-classification.tex <==
One can classify the state being retained in the network's middleboxes based on the broad approach outlined in Split-Merge~\cite{Rajagopalan:2013:SSS:2482626.2482649}:

There is state that is {\em internal} to the host that the NF resides in. This internal state includes the occupancy of the queues, the utilization of the host platform including the various OS processes that may be running, the information that is currently cached at the node etc. Some of this internal state may be transient in nature.

A second component of internal state would be the state that is available in the manager of the NFs. In our SDNFV framework, we have the NF manager retaining state associated with the tasks that have been assigned to the NFs on the host as well as the packets and tasks that are queued for the NFs that are instantiated on the host. The NF manager may also be aware of a service chain (or the portion of the service chain) that is instantiated on the host.

There is {\em external} network-related state that is related to the protocol and state that influences how packets are treated in the network. Some of this state has to be consistent across NF instances in the network, or even across different NFs that are involved in handling flows in the network. ~\cite{Rajagopalan:2013:SSS:2482626.2482649} classifies these as ``Coherent" external state.
Another component of external network-related state are those that may be distributed across various NFs, independent of whether they are across replicas of the same NF or if they are for a distinct NF. These include the entries in flow tables as well as timers.

The hierarchical control framework we propose can base its decision on both internal host state as well as the external network-related state.

%High level: Two types: Internal and External.
%Internal: pertinent only to replica and considered ephemeral. Ex. OS processes, cache.
%External: That needs to be transferred and synchronized. Two types Coherent and Partitioned.
%Coherent: that needs to be consistent across all the replicas. Ex. Counters.
%Partitioned: split among replicas. Ex. Flow tables, timers.

In contrast to our approach of having a hierarchical control, OpenNF retains the internal host state in an NF state manager as well as the network-related state  in the Flow Manager. Both of these components are reatined in the logically centralized OpenNF Controller and thus may suffer from the same scalability as a OpenFlow central controller.

